Cloud-Based Video Streaming Services: A Survey

Video streaming, in various forms of video on demand (VOD), live, and 360 degree streaming, has grown dramatically during the past few years. In comparison to traditional cable broadcasters whose contents can only be watched on TVs, video streaming is ubiquitous and viewers can flexibly watch the video contents on various devices, ranging from smart-phones to laptops and large TV screens. Such ubiquity and flexibility are enabled by interweaving multiple technologies, such as video compression, cloud computing, content delivery networks, and several other technologies. As video streaming gains more popularity and dominates the Internet traffic, it is essential to understand the way it operates and the interplay of different technologies involved in it. Accordingly, the first goal of this paper is to unveil sophisticated processes to deliver a raw captured video to viewers' devices. In particular, we elaborate on the video encoding, transcoding, packaging, encryption, and delivery processes. We survey recent efforts in academia and industry to enhance these processes. As video streaming industry is increasingly becoming reliant on cloud computing, the second goal of this survey is to explore and survey the ways cloud services are utilized to enable video streaming services. The third goal of the study is to position the undertaken research works in cloud-based video streaming and identify challenges that need to be obviated in future to advance cloud-based video streaming industry to a more flexible and user-centric service.

==> Jason_streaming_types.tex <==
\section{Video Streaming Types}
We consider two main categories of video streaming based on the video origin and time of recording: video-on-demand (VOD) and live-streaming.  Video-on-demand (VOD) describes a scenario in which an archived video that was previously recorded is streamed to another computer, while live streaming involves a video that is not archived and is recorded at the time of streaming.  While the end-user experience may be similar for each, here are several important differences in their implementation.

%Talk about cardinality...
Both categories have similar cardinalities, though what the cardinaility means can differ. VOD is primarily done in a one-to-many context, in which the video file is hosted on a single server and is streamed to many viewers (e.g. YouTube). These systems, however, incur large costs to the server. This can be remedied using a many-to-many, peer-to-peer filesharing approach to streaming \cite{liu:p2pstreaming}.

Live-streaming is most commonly done through a peer-to-peer framework to cut out need for an external server. Different types of live-streaming can be further categorized by the quantity of streamers and viewers.  The simplest case is one-to-one streaming, which occurs in a two-person video chat (e.g. Skype).  Similarly, many-to-many streaming can occur in group chats consisting of more than two people.  One-to-many streaming occurs when a single camera or source streams to many viewers, (e.g. live television broadcasts).  Finally, many-to-one streaming describes many cameras streaming to a single device (e.g. a video surveillance system).

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{fig/streaming_types}
    \caption{A taxonomy of streaming types considered by this work}
    \label{fig:stream_types}
\end{figure}
%Talk about buffer size...
%The experience of each streaming category is heavily affected by buffer sizes \cite{stypes:thesis}.  Because videos-on-demand are archived and there is typically no desire to keep the time in sync with another participant, the buffer size can be as large as the viewing hardware will allow.  This allows high quality frames to be built up, and leaves remaining frames if there is a drop in service on either end.  Live-streamed video typically demands the viewer to keep within a small number of seconds of the streamer, thus demanding a small buffer size.  For one-to-many communication, such as live event broadcasting, several seconds of delay are often tolerated, as the communication is only going one-way.  However, for streaming that involves two-way communication (individual or group chat), latency must be reduced to the smallest amount possible to maintain natural human communication with minimal interruptions.  This requires a very small buffer, so that frames are displayed more quickly, and often necessitates lower quality video.

%Talk about asynchronous interactive video
Another unusual type of video streaming that has recently increased in popularity is a method we will term \emph{asynchronous interactive video streaming}.  This method is used for applications such as online games or video processing \cite{vstypes:gaming}, which may be performed on machines that are ill-equipped to handle the processing load required by the application, but are able to receive a video stream.  Using this architecture, a client will send their input data to a cloud server supplied by the service provider, which will perform any necessary input handling and parsing, update the interactive graphics, and send the video to the client as a stream.  The result, to the client, is similar to an interactive live stream.

%Each type of streaming faces its own challenges which are described in the coming sections.


==> how_vs_work.tex <==
\section{How Video Streaming Work}\label{sec:hvsw}
To stream a VOD or live video, it basically has to go through three main modules: \emph{video encoding/transcoding, video packaging, }and \emph{delivery network}, as shown in Figure~\ref{fig:achitecture}

\begin{figure}[htb] 
    \centering
    \includegraphics[width=5.5in]{streaming_flow}
    \caption{Workflow of processes for video streaming.}
    \label{fig:achitecture}
\end{figure}

As most devices nowadays can take HD or even 4K video contents, a raw recorded video content takes GBs or TBs of storage, which makes it difficult to store, not to mention streaming it over the Internet. However, the concept of a video is just continuously showing a group of pictures at a certain rate. It usually contains spatial and temporal redundancy inside a frame or between successive frames, respectively. To compress a video, we have to remove these redundancies with one of the available compression standards, \eg H.274/AVC~\cite{schwarz2007overview}, VP9~\cite{mukherjee2013latest}, and HEVC~\cite{intro_3} \etc. The whole process is called video encoding. Based on these standards (codec), the original video is encoded to a specific compressing standard (codec), resolution, bit rate and frame rate at a much smaller size.

However, considering the diversity of viewing devices (e.g mobile phone, laptop, television) on the market under different Internet access ability, a video with only one specific codec, resolution, bit rate and frame rate cannot possibly be played on all devices. To meet such diverse demands, an encoded video has to be converted (transcoded) to different versions, to produce multiple codec, resolution, bit rate and frame rate videos. Video transcoding will be discussed in Section~\ref{sec:video_transcoding} with more details.


With all different transcoded renditions, however, the videos still cannot be played on viewers' devices. They still need a specific container format (\eg .mp4, .avi, .flv) that supported by the player. While for streaming, ISOBMFF ~\cite{timmerer2010http} based mp4 format and 3GPP TS~\cite{} based ts format which is widely used in MPEG2 transport stream. Inside these container format headers, it specifies the supported streaming protocols and the rules to send video chunks. On the other layer, in order to stream the video through the Internet, we have to obey different kind of Internet protocols, \eg HTTP~\cite{fielding1999hypertext}, RTMP~\cite{lesser2005programming}, and RTSP~\cite{schulzrinne1998real} \etc which are used in different streaming protocols. The whole process is called: video packaging, more details will be discussed in Section~\ref{sec:video_packaging}.

After packaging, a video is able to be streamed and played whenever it is requested by viewers. However, due to Internet transmission delay, it can cause viewers far away from a server to suffer long startup time. To reduce this delay, an edge server containing the video content should be placed near different user locations. Content delivery network (CDN) ~\cite{buyya2008content} plays an important role in resolving this issue, which is utilized to cache video contents at edge servers where near viewers at different geological locations. Another option is no central servers, but utilizing each receiver (\eg viewer's computer) as a server as well to send video contents to another receiver, this is called P2P~\cite{ramzan2012video}. More details of the delivery network will be discussed in Section~\ref{sec:delivery_content}


With the development of video streaming, other topics like video encryption, analysis and storage efficiency becomes important as well. They will be discussed in Section~\ref{sec:security}, Section~\ref{sec:analysis} and Section~\ref{sec:storage}, respectively.



==> references.tex <==
\begin{frontmatter}
\chapter*{References}
\end{frontmatter}

\begin{thebibliography}{10}

\bibitem{Arnold74}
V.~I. {Arnol'd}.
\newblock {The asymptotic Hopf invariant and its applications}.
\newblock In {\em Proc. Summer School in Differential Equations}, pages
  133--148, 1974.

\bibitem{Berger84}
M.~A. {Berger}.
\newblock {Rigorous new limits on magnetic helicity dissipation in the solar
  corona}.
\newblock {\em Geophys. Astrophys. Fluid. Dyn.}, 30:79--104, 1984.

\bibitem{Berger99a}
M.~A. {Berger}.
\newblock {Magnetic Helicity in Space Physics}.
\newblock In M.R. {Brown}, R.C. {Canfield}, and A.A. {Pevtsov}, editors, {\em
  Magnetic Helicity in Space and Laboratory Plasmas}, pages 1--9. Geophys.
  Monogr. Ser. 111, AGU, 1999.

\bibitem{Berger03}
M.~A. {Berger}.
\newblock {Topological quantities in magnetohydrodynamics}.
\newblock In A.~{Ferriz-Mas} and M.~{N{\'u}{\~n}ez}, editors, {\em Advances in
  Nonlinear Dynamics}, pages 345--383. Taylor and Francis Group, London, 2003.

\bibitem{BergerF84}
M.~A. {Berger} and G.~B. {Field}.
\newblock {The topological properties of magnetic helicity}.
\newblock {\em J. Fluid. Mech.}, 147:133--148, 1984.

\bibitem{Brandenburg01}
A.~{Brandenburg}.
\newblock {The Inverse Cascade and Nonlinear Alpha-Effect in Simulations of
  Isotropic Helical Hydromagnetic Turbulence}.
\newblock {\em Journal title}, 550:824--840, 2001.

\bibitem{Brown99}
M.R. {Brown}, R.C. {Canfield}, and A.A. {Pevtsov}.
\newblock {\em {Magnetic Helicity in Space and Laboratory Plasmas}}.
\newblock Geophy. Mon. Ser. 111, AGU, 1999.

\bibitem{Chae04}
J.~{Chae}, Y.-J. {Moon}, and Y.-D. {Park}.
\newblock {Determination of magnetic helicity content of solar active regions
  from SOHO/MDI magnetograms}.
\newblock {\em Solar Physics}, 223:39--55, 2004.

\bibitem{Dupont07}
J.-C. {Dupont}, F.~{Schmidt}, and P.~{Koutny}.
\newblock {An example of reference with BibTeX}.
\newblock {\em Solar Physics}, 323:965--985, 2007.

\bibitem{Elsasser56}
W.~M. {Elsasser}.
\newblock {Hydromagnetic Dynamo Theory}.
\newblock {\em Rev. Mod. Phys.}, 28:135--163, 1956.

\bibitem{Heyvaerts84}
J.~{Heyvaerts} and E.~R. {Priest}.
\newblock {Coronal heating by reconnection in DC current systems - A theory
  based on Taylor's hypothesis}.
\newblock {\em Journal title}, 137:63--78, 1984.

\bibitem{Kusano04}
K.~{Kusano}, T.~{Maeshiro}, T.~{Yokoyama}, and T.~{Sakurai}.
\newblock {The Trigger Mechanism of Solar Flares in a Coronal Arcade with
  Reversed Magnetic Shear}.
\newblock {\em Journal title}, 610:537--549, 2004.

\bibitem{Low97}
B.~C. {Low}.
\newblock {The role of coronal mass ejections in solar activity}.
\newblock In N.~{Crooker}, J.~A. {Joselyn}, and J.~{Feynman}, editors, {\em
  Coronal Mass Ejection}, pages 39--48. Geophys. Monogr. Ser. 99, AGU, 1997.

\bibitem{Mandrini05}
C.~H. {Mandrini}, S.~{Pohjolainen}, S.~{Dasso}, L.~M. {Green},
  P.~{D{\'e}moulin}, L.~{van Driel-Gesztelyi}, C.~{Copperwheat}, and
  C.~{Foley}.
\newblock {Interplanetary flux rope ejected from an X-ray bright point. The
  smallest magnetic cloud source-region ever observed}.
\newblock {\em Journal title}, 434:725--740, 2005.

\bibitem{Melrose04}
D.~{Melrose}.
\newblock {Conservation of both current and helicity in a quadrupolar model for
  solar flares}.
\newblock {\em Solar Physics}, 221:121--133, May 2004.

\bibitem{Moffatt69}
H.~K. {Moffatt}.
\newblock {The degree of knottedness of tangled vortex lines}.
\newblock {\em J. Fluid Mech.}, 35:117--129, 1969.

\bibitem{Nindos03}
A.~{Nindos}, J.~{Zhang}, and H.~{Zhang}.
\newblock {The Magnetic Helicity Budget of Solar Active Regions and Coronal
  Mass Ejections}.
\newblock {\em Journal title}, 594:1033--1048, 2003.

\bibitem{Pariat05}
E.~{Pariat}, P.~{D{\'e}moulin}, and M.~A. {Berger}.
\newblock {Photospheric flux density of magnetic helicity}.
\newblock {\em Journal titl}, 439:1191--1203, 2005.

\bibitem{Rust94}
D.~M. {Rust}.
\newblock {Spawning and shedding helical magnetic fields in the solar
  atmosphere}.
\newblock {\em Journal title}, 21:241--244, 1994.
\end{thebibliography}

==> streaming_protocol.tex <==
\subsubsection{Streaming Protocol}~\label{streaming_protocol}
\noindent\textbf{HTTP}
With this as background, let’s start examining the application-layer protocols used to stream video, starting with the granddaddy of them all, HTTP. As you probably know, HTTP stands for Hypertext Transfer Protocol, which is the lingua franca for the web. HTTP governs the communications between web servers and browsers and is the protocol used to distribute all the content on websites to remote viewers, including HTML text, GIF and JPG graphics, PDF files, and other web-based (as opposed to FTP) downloads.

Early experiments with delivering video via HTTP were less than satisfactory for some reasons, not the least of which was the limited bandwidth available in the 28/56Kbps modems of the day. The first video files posted on the web were delivered via download and play, which mean they had to be fully downloaded before playback began. Then Apple pioneered the concept of progressive download, where the video could start to play as it was downloaded, which helped a bit, but didn’t provide functionality like lookahead seeking or random access.

The other big negatives of the HTTP-delivered video were cost and quality of service issues. HTTP delivery is accomplished as fast as available bandwidth will allow. If a viewer connected via a high-speed connection, the entire video file was sent as quickly as possible. If the viewer stopped watching after a few moments, much of that transfer was wasted.

In addition, this mode of delivery made it difficult to serve multiple viewers. When viewer A clicked on the video, the server started sending the video as quickly as possible. When viewers B, C, D, and E clicked on the video, outbound bandwidth might be insufficient to serve them any video until the transfer to viewer A was complete.

\noindent\textbf{RTP}
As streaming media increased in importance, several streaming protocols were created to address these issues, including the aforementioned RTSP, Microsoft Media Services (MMS) and Macromedia’s (and then Adobe’s) Real-Time Messaging protocol (RTMP). At a high level, these protocols shared several common complete.

First was the existence of a streaming server, or a software program charged solely with delivering streaming content. These streaming servers worked in conjunction with traditional HTTP servers so that when a viewer clicked a link on the HTTP server, it initiated a connection between the streaming server and the player that persisted until the viewer stopped watching. Because of this connection, these protocols are considered “stateful,” as compared to HTTP, which is stateless and has no connection between server and player. 



\subsubsection{Streaming Technologies}
\noindent\textbf{Progressive Download}
In the old days, a file will not play until it is completely downloaded, which means the user has to wait for a long time before beginning watch the video. Progressive downloading solves this problem to allow video to be played prior to the completion of the full download. Video files are split into small chunks, which will be downloaded linearly. 

The drawback of progressive downloading is that it has less flexibility. The user can not move forward if until that chunk of the video is downloaded. On the other hand, if the user stops watch the video, the remaining parts of the downloaded video are wasted, results in unnecessary bandwidth. Another concern is that copyright, since the full video will be downloaded on the user's hard drive.

\noindent\textbf{Streaming}

To resolve the issue of progress download, streaming becomes thriving; the typical example is Adobe flash. Streaming technology is based on real-time protocol (RTP), that means server and client keep communicate with each other. It gives the user much more flexibility to skip some video chunks and moving forward because the streaming server will send the client the right chunk of video based on the user's request. Also, streaming only delivers content until the user abandons viewing the content, which avoids wasting bandwidth. One other efficiency in streaming is that video files are only cached in viewer's device and will be automatically removed after watching. Therefore, it saves viewer hard drive storage as well as protecting the copyright.

However, RTP-based streaming technology has a major drawback that it is using a different port from HTTP, which causes streaming may be blocked by the firewall of viewer's devices. Also, an extra plugin may need to be able to stream, \eg Adobe Flash plugin. It decreases the mobility of streaming technology, especially nowadays Apple mobile devices has stopped supporting flash.

\noindent\textbf{Adaptive Streaming} 







Choosing a streaming technology involves multiple considerations, including an understanding of the pluses and minuses of the streaming protocol used by the technology. Communications protocols are rules governing how data is communicated, defining elements like the syntax of file headers and data, authentication, and error handling. There are easily dozens of protocols involved in sending a simple data packet over the internet, and it’s important to understand how they work together. All streaming protocols are in the application layer, which means they can use any layer beneath it for plumbing functions like transmitting data packets. 

For example, the Real Time Streaming Protocol (RTSP) is an application-level streaming protocol that can use multiple protocols in the transport layer to transmit its packets, including the Universal Datagram Protocol (UDP) and Transmission Control Protocol (TCP). Sometimes application-level protocols are written specifically for a particular transport protocol, like the Real-Time Transport Protocol (RTP), which is typically built on UDP transport.

Hopefully, this brief overview will help you understand where streaming protocols live and how they interact with other, lower level protocols. This is as technical as we get, folks, so from here on out it should be smooth sailing.

\subsubsection{HTTP}
With this as background, let’s start examining the application-layer protocols used to stream video, starting with the granddaddy of them all, HTTP. As you probably know, HTTP stands for Hypertext Transfer Protocol, which is the lingua franca for the web. HTTP governs the communications between web servers and browsers and is the protocol used to distribute all the content on websites to remote viewers, including HTML text, GIF and JPG graphics, PDF files, and other web-based (as opposed to FTP) downloads.

Early experiments with delivering video via HTTP were less than satisfactory for a number of reasons, not the least of which was the limited bandwidth available in the 28/56Kbps modems of the day. The first video files posted on the web were delivered via download and play, which mean they had to be fully downloaded before playback began. Then Apple pioneered the concept of progressive download, where the video could start to play as it was downloaded, which helped a bit, but didn’t provide functionality like lookahead seeking or random access.

The other big negatives of the HTTP-delivered video were cost and quality of service issues. HTTP delivery is accomplished as fast as available bandwidth will allow. If a viewer connected via a high-speed connection, the entire video file was sent as quickly as possible. If the viewer stopped watching after a few moments, much of that transfer was wasted.

In addition, this mode of delivery made it difficult to serve multiple viewers. When viewer A clicked on the video, the server started sending the video as quickly as possible. When viewers B, C, D, and E clicked on the video, outbound bandwidth might be insufficient to serve them any video until the transfer to viewer A was complete.

\subsubsection{The Rise of Streaming Protocols}
As streaming media increased in importance, several streaming protocols were created to address these issues, including the aforementioned RTSP, Microsoft Media Services (MMS) and Macromedia’s (and then Adobe’s) Real-Time Messaging protocol (RTMP). At a high level, these protocols shared several common complete.

First was the existence of a streaming server, or a software program charged solely with delivering streaming content. These streaming servers worked in conjunction with traditional HTTP servers so that when a viewer clicked a link on the HTTP server, it initiated a connection between the streaming server and the player that persisted until the viewer stopped watching. Because of this connection, these protocols are considered “stateful,” as compared to HTTP, which is stateless and has no connection between server and player. 

This connection addressed most of the negatives of HTTP delivery. Streaming protocols enabled seeking to random points in the video file, and adaptive streaming, where multiple encoded files could be distributed to the player based upon available bandwidth and CPU power. The server could meter out the flow of video to the player on a just in time basis, so if the viewer stopped watching, little extra bandwidth was wasted. Because the outbound flow was metered, a streaming server could more effectively serve multiple users, improving the overall quality of service.

\subsubsection{HTTP - Back to the Future}
Over time, as Flash video rose to dominate the streaming video landscape, RTMP became the dominant streaming protocol and is still widely used today. However, with the introduction of Microsoft’s HTTP-based Smooth Streaming and Apple’s HTTP Live Streaming (HLS), HTTP-based streaming technologies began a resurgence for multiple reasons, both having to do with perceived negatives of RTMP and innovations in HTTP technologies that addressed many of its negatives.

Perceived shortcomings in RTMP include:

RTMP packets may be blocked by certain firewalls, though the Adobe Media Server has workarounds if these problems are experienced.

RTMP packets can’t leverage standard HTTP caching mechanisms available within the networks of ISPs, corporations, and other organizations, which can improve distribution efficiency and quality of service.

The persistent server to a player connection means increased costs because streaming servers cost money.

The required server may also limit scalability as compared to HTTP-based streaming since there are many more HTTP servers than RTMP.

I say "perceived," because as this article is being written (August 2012), RTMP is still used by sites like Bloomberg and The Street.com, which tends to cast doubt on the notion that RTMP can’t get through to heavily firewalled viewers. ESPN and MTV also use RTMP, which makes you question the scalability and cost issues.

These doubts aside, there’s a general perception among technical cognoscenti that HTTP-based technologies are more effective at delivering high-quality streams. Plus, Adobe introduced HTTP Dynamic Streaming (HDS) in 2010, providing a Flash-based alternative for those seeking HTTP-based streaming to the desktop. All of a sudden, changing to HTTP-based online video delivery no longer involved a seismic shift to a totally new technology; Flash users could continue to leverage their investment in Flash development and infrastructure and leverage the benefits of HTTP streaming.

As mentioned, several innovations in HTTP streaming also addressed previous limits of the technology. As before, there is no persistent connection between the server and the player; the video resides on any HTTP server, and the technology remains stateless. However, now all HTTP-based streams are broken into chunks, either separate files or segments within a larger file. Rather than retrieving a single large file with a single request, HTTP-based technologies retrieve consecutive short chunks on as needed basis.

This has multiple benefits. First, there’s little waste because the video is delivered as it is watched. This effectively meters out the video, enabling a single HTTP server to efficiently serve more streams. Seeking is no problem; if the viewer drags the playhead forward, the player can just retrieve the appropriate chunks. These technologies also enable the efficient switching between streams, so all the listed technologies (Smooth Streaming, HLS, and HDS) stream adaptively.

Since these technologies are delivered via HTTP, they sidestep the issues faced by RTMP. HTTP-based technologies are firewall friendly and can leverage HTTP caching mechanisms. Because no streaming server is required, they are less expensive to implement and can scale more cheaply and effectively to serve available users.

\subsubsection{Final Points}
Again, RTMP distribution is still widely and beneficially used by many websites today. However, while there may be little impetus for some sites to change, at this point if you’re considering a streaming technology, the overwhelming sentiment is to deliver via HTTP. Of course, for adaptive delivery to Apple devices (and Android 3.0 and higher), HLS is your only option.

It’s also useful to recognize that most video content is delivered via plain old HTTP progressive download. Sure, there are limitations, like the lack of adaptive streaming, but you can’t say it’s worked out too badly for YouTube, who delivers about 70\% of video over the web, exclusively via progressive download. However, this approach prevents YouTube from deploying the digital rights management (DRM) techniques available via HDS, Smooth Streaming, and HLS to protect their videos, which is a key reason sites with branded content using these technologies.

Finally, the focus of this article has been general internet streaming. Particularly for intranet use, streaming-server-based protocols like IP Multicast and applications like peer-to-peer delivery provide lots of value and even more promise. So don’t throw out the baby with the bathwater; streaming servers aren’t “bad” and HTTP isn't "good." Rather, choose the best tool for the job.
